Compression of GPS Trajectories using Autoencoders

The ubiquitous availability of mobile devices capable of location tracking led to a significant rise in the collection of GPS data. Several compression methods have been developed in order to reduce the amount of storage needed while keeping the important information. In this paper, we present an lstm-autoencoder based approach in order to compress and reconstruct GPS trajectories, which is evaluated on both a gaming and real-world dataset. We consider various compression ratios and trajectory lengths. The performance is compared to other trajectory compression algorithms, i.e., Douglas-Peucker. Overall, the results indicate that our approach outperforms Douglas-Peucker significantly in terms of the discrete Fr\'echet distance and dynamic time warping. Furthermore, by reconstructing every point lossy, the proposed methodology offers multiple advantages over traditional methods.

==> text/Methodology__Kopie_.tex <==
\chapter{Methodology}\label{sec:Methodology}
After the previous introduction to the domain of (GPS-)trajectories and the
following foundations regarding autoencoders and LSTMs, a new method for
trajectory compression is presented in this chapter. After a short presentation
of the two datasets that are used in this thesis and a description how the data
is prepared, the autoencoder architecture for trajectory compression is
introduced. Furthermore methods used for performance evaluation are presented
based on the metrics explained in section \ref{sec:metrics}.

\section{Datasets}\label{sec:datasets}
In order to compare the compression model presented in this thesis to
traditional line simplification methods, two datasets are used. Both consist of
multiple recorded trajectories but vary in data structure and origin. The
origin, differences and use cases of those datasets are presented in this
section.

\subsection{Quake III Dataset}
The first considered dataset consists of trajectories recorded in Quake III
Arena, a popular first-person shooter video game (\cite{Breining2011}). Since
the user can move inside a fixed three dimensional area, the trajectories of
the player are series of three-dimensional positions that can be used to place
the user in Euclidean space. Those points are recorded at each position update
of the game which is circa every 33 ms (based on an frame rate of 30 fps). The
sampling rate of the positions is therefore far higher than it is reasonable in
real life scenarios with GPS. Furthermore, the positions are recorded from the
game directly, so that the uncertainty and inaccuracy of GPS is eliminated.
While GPS trajectories usually contain an explicit timestamp for each position,
the temporal information in this dataset is represented only implicitly through
the fixed sampling rate. Time information is therefore only available relative
to the start of the trajectory which is reasonable in the context of a
restricted environment like a match of a computer game. The data was recorded
in different scenarios and settings of the game and is stored in multiple log
files. Each run represents a trajectory from spawn to death. This dataset is
used for an evaluation for multiple reasons. First, it is an artificial dataset
with positions recorded directly from the game engine, so that the inaccuracy
of GPS is eliminated. Second, the amount of noise and inexplicable peaks is
lower than the later considered dataset. Furthermore, the sampling rate is
fixed and very high, so that visualizations are easily understandable and can
be used to find shortcomings of the model. All in all, many of the
environmental variables introduced through real life data are not present and
the dataset can be used for a first evaluation of trajectory compression. An
example trajectory from the Quake III dataset plotted in three-dimensional
Euclidean space is shown in figure \ref{fig:quake_traj}.

\begin{figure}[hpbt]
	\centering
	\includegraphics[width=\textwidth]{pictures/methodology/quake_traj2}%
	\caption{Example trajectory of the Quake III dataset.}
	\label{fig:quake_traj}%
\end{figure}

\subsection{T-Drive}
In 2010, Microsoft published a paper that uses a dataset of GPS trajectories
named T-Drive (\cite{Yuan2010}, \cite{Yuan2011}). The original dataset contains
the recorded trajectories of over 33,000 taxis in Beijing over the course of
three months and has become one of the standard datasets for researchers that
work with GPS trajectory data. Parts of this dataset were made public and are
used in this thesis to train the autoencoder model and compare it to existing
methods. The available data contains real trajectories of more than 10,000
taxis over the course of one week in 2009. Around 9 million driven kilometers
were tracked by 15 million sample points. The data is available as CSV files
where each data point contains a taxi ID, a timestamp and the position of the
car in latitude/longitude representation. This dataset is used to evaluate the
here proposed model on real life data. The duration between two samples lasts
from few seconds to multiple hours, but there are also duplicates in the
dataset. Due to those inconsistencies and noise, the data has to be
preprocessed before it can be used. The steps taken in order to work with
T-Drive are presented in the following section \ref{sec:preprocessing}. An
example trajectory projected on a map is shown in Figure \ref{fig:tdrive_traj}.
Map information is based on \cite{OpenStreetMap2017}, the map style and design
is from \cite{Carto2017}. The trajectory is treated as polyline so that the
data between recorded points can be interpolated linearly. Here one of the main
disadvantages of the usual trajectory representation is visible. The line
segments between vertices cross buildings and parks so a route is shown that
taxis obviously could not take. Due to the low sampling rate, the positions
between records can only be assumed by interpolation or map matching if a road
network is available. In contrast to the Quake dataset, the positions are
two-dimensional and are accompanied by a timestamp. In this case the knowledge
of the absolute point in time offers important information since the sample
rate is not as accurate as in the Quake dataset and the information can be used
for example to analyze hotspots during rush hour.

\begin{figure}[hpbt]
	\centering
	\includegraphics[width=\textwidth]{pictures/methodology/tdrive_traj}%
	\caption{Example trajectory of the T-Drive dataset.}
	\label{fig:tdrive_traj}%
\end{figure}

\section{Data Preparation}
When neural networks are applied to data, one of the key factors to obtain
successful results, is good data preparation. The used activation functions
usually expect a certain range of values like $[-1, 1]$ or $[0, 1]$. Since
autoencoders also exploit the present redundancies and patterns in data to
learn useful features, the data has to be prepared before it is fed to the
network.

\subsection{Preprocessing of T-Drive}\label{sec:preprocessing}
The T-Drive dataset is a collection of real life trajectories recorded by GPS
receivers inside taxis. Because of effects like urban canyons where tall
buildings on the sides of a street affect the GPS signal reception, the data
suffers inconsistencies and random peaks. This noise has to be eliminated in a
preprocessing step to make the results of the evaluated methods comparable.
All points with the same taxi ID make up a trajectory that is further
processed. Only points that are in the metropolitan area of Beijing are
considered, so that obvious noise like points on latitude zero and longitude
zero are removed early in the preprocessing. As a first step it is ensured that
the timestamps of the points in a trajectory are continuously increasing.
Therefore points are eliminated if their timestamp is less than or equal to the
last sampled timestamp.

Some of the taxi recordings have gaps of multiple hours in the data which
indicates that the taxi was not used in the meantime and no data was recorded
during that time. Therefore the trajectory of a taxi ID is split if consecutive
points are more than two hours apart. While parts of the taxis stopped
recording during those idle times, other receivers continued recording
resulting in multiple continuous samples around the same position.
Interestingly those positions are not exactly the same all the time, which is
attributable to inaccuracies of the GPS tracker. The idle times should be
removed from the data since they add no informational value to the data.
However, not all points on the same position should be removed, because it is
possible that the taxi just has to wait at a traffic light or is in a traffic
jam. Therefore the speed between consecutive points is calculated. Since the
positions are stored as latitude and longitude, the distance between two points
is calculated by the haversine formula introduced in section
\ref{subsec:point_distances}.

Based on the spatial distance and the temporal duration between two points, the
speed can be calculated under the assumption that it is constant between two
points. It is assumed, that the taxi is idle, if it stays below 1 m/s for more
than 10 sample points. If it is idle, those points are removed and the
trajectory is split in two parts. Based on the speed it is also possible to
remove outliers that are probably introduced by technical errors. Therefore the
trajectory is also split if the speed between two points is greater than 55
m/s. The values and constants used were chosen by trial and error and common
sense. E.g. it is not realistic, that a taxi drives with 198 km/h through
Beijing as the crow flies. The steps taken to preprocess the data only ensure
that the most extreme inconsistencies are removed, while the level of
inaccuracy due to technical limitations stays realistic. The result is
therefore a set of trajectories with different numbers of time steps, that
represent realistic movements of cars over time.\medbreak

Since the trajectories in the Quake III dataset are recorded directly from the
game, the level of inaccuracy is low and there is no further preprocessing
applied. Each run between spawn and death makes up a trajectory with different
numbers of time steps.

\subsection{Generation of Training Data}
In order to evaluate the performance of a neural network the available dataset
has to be split up in two parts. The majority of the data is used for training
while a smaller part is used to evaluate the accuracy of the network output.
Since the test part is not used for training, it can be evaluated how well the
model generalizes to new data. This is crucial because an autoencoder tends to
overfit on the reconstruction of the training data which leads to a bad
performance for new data. The structure and properties of the two considered
datasets are different, hence the model is trained and evaluated independently
for both. The following description of normalization and generation of data for
the training phase is applied to both sets.

The trajectories of the dataset are split into two parts. One contains around
90\% of the recorded points and is used for training the model. The remaining
trajectories that contain around 10\% of the points are used to test and
validate the model. The trajectories obtained after the preprocessing steps
consist of varying numbers of time steps. Since the goal of this thesis is to
evaluate the feasibility of autoencoder approaches for trajectory compression
in general, the additional complexity of variable trajectory lengths is
removed. Nonetheless, different sequence lengths of trajectories should be
evaluated. For this reason the two sequence lengths $|T| = 20$ and $|T| = 40$
are considered. The available trajectories are therefore split into chunks of
20 and 40 time steps respectively.

The performance of a neural network is strongly dependent on the available data
during the training phase since the optimal weights are learned based on this
data. To increase the amount of training data, a sliding window approach is
applied on the trajectories. If a trajectory consists of more time steps than
the required sequence length $|T|$, the first $|T|$ points $(P_{1}, ...,
P_{|T|})$ are added to the training data as input sequence. Afterwards the
sliding window is shifted by one so that the steps $(P_{2}, ..., P_{|T|+1})$
build the next input sequence. This procedure is subsequently repeated until
the end of the trajectory is reached. Through this approach, the number of
sequences to train the model can be enlarged from several thousands to a few
million. The trajectories used for testing are not further manipulated but also
split into chunks of 20 respectively 40 steps.

\subsection{Normalization}
Another important step in the preparation of data for an autoencoder is the
normalization. Similarities between trajectories are often based on the form of
the route they describe rather than their absolute position in space. Rescaling
each trajectory to values between 0 and 1 therefore takes complexity out of the
network which leads to better performance and shorter learning time. For each
dimension, the minimum value (offset) and the scaling factor of a trajectory
are saved. The compressed trajectory therefore consists of the output of the
encoder network and the information to rescale the trajectory to its original
domain. After decoding the latent representation, the trajectory can be put to
its absolute position with those rescaling and offset values. The autoencoder
therefore just has to learn the relative distances between the points of the
trajectory and no absolute values.

\section{Autoencoder Architecture}\label{sec:architecture}
The main goal of this thesis is to demonstrate the feasibility of autoencoder
networks to compress and reconstruct (GPS-)trajectories and evaluate their
performance compared to traditional handcrafted compression methods. Since the
trajectory of a moving object is usually represented as a time series of
discrete positions annotated with a timestamp, a Recurrent Neural Network is
used to build the autoencoder. More precisely the Long Short-Term Memory
Network architecture builds the core of the model because of its remarkable
performance in classification and prediction tasks with time series data.

\subsection{Encoder}

\begin{figure}[bt]
	\centering
	\includegraphics[width=\textwidth]{pictures/methodology/encoder}%
	\caption{Schematic of the LSTM encoder.}
	\label{fig:encoder}%
\end{figure}

A LSTM cell builds the basis of the encoder that transforms the input
trajectory into a lower-dimensional latent representation. At each time step a
data point of the trajectory is fed to and processed by the LSTM. Depending on
which of the datasets described in section \ref{sec:datasets} is used, the
three dimensions represent the position of an object inside a three-dimensional
space or a two-dimensional position and a timestamp respectively. While it
would be possible to use a variable number of time steps per sequence, the
length of the trajectory $|T|$ is fixed beforehand in order to reduce
complexity. The output at every time step but the last is discarded. Only the
output of the final step is used as it contains the encoded information of the
whole trajectory including the temporal dependencies. This latent
representation forms together with the scaling and offset value from the
normalization step the compressed version of the original trajectory. Per
trajectory and feature two rescaling values for absolute position and scaling
factor are needed so that six values are already set for the compressed
trajectory. The number of values in the original trajectory are $|T| \cdot 3$,
since there are three values for each point in the trajectory. All the points
of the trajectories as well as the rescaling values and the latent variable of
the autoencoder are stored in 32 bit each, so that the number of values in the
original and compressed representation can be directly used to calculate the
compression ratio. Since the size of an input trajectory and the size of the
rescaling values are set, the compression ratio can be adjusted by modifying
the dimensionality of the encoder LSTM output and therefore the latent variable
of the autoencoder. The compressed size is the sum of the numbers of latent and
rescale values.  Figure \ref{fig:encoder} shows a schematic of the unrolled
LSTM encoder that maps a trajectory into the latent space.

\subsection{Decoder}
Similar to the encoder, the decoder also consists of a LSTM cell. This part of
the autoencoder maps the latent variable back to the original space. At
each time step the latent variable is fed again to the network as its input and
the resulting output represents the reconstructed three-dimensional data point.
During the training process of a neural network the weights are optimized in
order to produce the expected output and learn generalizable features of the
given data. The ability to perform as expected is therefore strongly dependent
on the number of weights available to optimize. This number of weights in
a LSTM is dependent on the dimensionality of the input and output data. Since
the weights are reused at each time step, the length of the sequence does not
influence this number. Compared to other tasks like image compression or
natural language generation, the trajectory data used in this use case is very
low-dimensional. For example, with a sequence length of 20 and a compression
ratio of 4, the latent variable has $\frac{20 \cdot 3}{4} - 6 = 9$ dimensions.
Therefore the input size of the decoder at each time step is 9 and the output
size is 3, since each point of the trajectory is three-dimensional. The number
of weights $n_{W}$ available in the cell is dependent on the number of neural
layers that are used. In a LSTM cell, the gates are implemented as neural
layers and the block input as well as the output is activated with a layer. The
number of weights can therefore be calculated by following formula:

$$
n_{W} =
4 \cdot ((n_{I} + 1) \cdot n_{O} + {n_{O}}^2)
$$

$n_{I}$ here is the input dimensionality and $n_{O}$ the output dimensionality.
The additional 1 is due to the bias term. The factor of four represents the
three gates of a LSTM and the input activation. In the example, the decoder
therefore would have only 156 weights available to fit to the data. For a
complex task like the trajectory reconstruction this would be far too little
parameters to achieve decent results. The output dimensionality of the decoder
is therefore set to 100, so that there are enough parameters that can be
adjusted to fit the temporal dependencies between points and produce good
results. In order to reduce the output back to a three dimensional space, a
fully connected layer with three output neurons is added at the LSTM
output. Figure \ref{fig:decoder} shows the architecture of the decoder.
\cite{Sutskever2014} stated that the performance of Sequence to Sequence
Autoencoders can be improved significantly, if the input sequence is reversed
before it is fed to the network. The target sequence stays in the original
order nonetheless. While no final explanation for this phenomenon could be
provided, the assumption is, that the introduction of more short-term
dependencies enables the network to learn better features. This method is
therefore also applied in the here proposed model.

\begin{figure}[hpbt]
	\centering
	\includegraphics[width=\textwidth]{pictures/methodology/decoder}%
	\caption{Schematic of the LSTM decoder.}
	\label{fig:decoder}%
\end{figure}

\subsection{Training Loss}\label{subsec:train_loss}
Autoencoders are usually trained with the mean squared error (MSE) as loss
function. For an $M$-dimensional expected point $P$ and its predicted
reconstruction $P'$ the MSE is defined as:

$$MSE(P, P') = \frac{1}{M}\sum_{m=1}^{M}(P'_{m} - P_{m})^2$$

This is generally a good fit, since unlike in classification tasks,
the input is also the target of the network. The values of input and output can
therefore be compared in a value-by-value fashion. Nonetheless MSE is a general
metric that doesn't incorporate domain knowledge in its error computation.

The trajectories of the Quake dataset are actually sequences of points in
three dimensional Euclidean space. Since the temporal dimension is only
implicitly available through the fixed sampling rate, solely the reconstruction
of the spatial information is important. Therefore, as alternative to MSE, the
actual Euclidean distance between a point and its reconstruction can be used as
loss metric.

$$d_{euc}(P, P') = \sqrt{\sum_{m=1}^{M}(P'_{m} - P_{m})^2}$$

The trajectories fed to and reconstructed by the neural network are however
normalized between 0 and 1. If the Euclidean loss is computed on those
normalized trajectories, the actual distances are hidden. Therefore the
training can be further improved by rescaling the original and reconstruction
before the loss calculation. \medbreak

The trajectories in the T-Drive dataset are represented in geo-coordinates
annotated with a timestamp. The temporal information is therefore explicitly
available. The error calculation based on the Euclidean distance would be
inaccurate since the coordinates are represented in latitude and longitude.
While the differences between the Euclidean distance and distances that
consider the spherical shape of earth are not significant for small areas, a
distance function like the haversine distance would be more general, more
accurate and more expressive. However, the computation of the haversine
distance is way more expensive than the Euclidean distance, while the
equirectangular approximation also presented in section
\ref{subsec:point_distances} offers a trade-off between both. Therefore, this
approximation is used to calculate the distance between the expected and the
predicted points. To incorporate the time in the loss function, the squared
error of this dimension is added to the loss.

\section{Performance Evaluation}\label{sec:evaluation}
In order to evaluate the performance of the previously proposed compression
approach, the autoencoder is compared to Douglas-Peucker. This algorithm is
widely used although it is not very enhanced. Since the goal of this thesis is
to evaluate whether autoencoders can be used for trajectory compression at all,
Douglas-Peucker provides a good baseline for comparison.

Every compression algorithm tries to optimize the trade-off between compression
ratio and reconstruction accuracy. Usually this optimization problem is
simplified by setting one of those parameters while the other is optimized.
One of the conceptual differences between Douglas-Peucker and the introduced
autoencoder approach is which parameter is set by the user or the application
in this trade-off. Douglas-Peucker is called with a fixed maximum error
tolerance value $\varepsilon$ regarding the spatial distance. If the removal of
a point doesn't introduce an error larger than $\varepsilon$ it is discarded.
The here proposed autoencoder encodes trajectories of a fixed size into a
predefined latent space, so that the compression ratio is set beforehand and
the autoencoder optimizes a function that minimizes the error between expected
and predicted trajectories.

For the comparison of the here introduced model with Douglas-Peucker, the
trajectories are split into chunks of fixed size and compressed with the same
compression ratio. Since the compression ratio can't be set directly as a
parameter with Douglas-Peucker, a $\varepsilon$ has to be found for each
trajectory, so that the compressed trajectories are comparable. This parameter
has to be evaluated for each sequence length and each compression ratio
separately. There are edge cases where no fitting $\varepsilon$ can be found,
since during the compression the distances of multiple points to the line
segments are the same. This means either all of those points have to be
discarded, leading to a higher compression ratio as targeted or all of those
points are kept in the compressed version so that the compression ratio is
lower than wanted. In such a case, a $\varepsilon$ providing the closest
compression ratio is selected and it is ensured that the mean compression ratio
over all trajectories doesn't significantly differ from the target.

Next to the fixed trade-off parameter, the autoencoder approach differs from
traditional compression approaches like Douglas-Peucker in the number of points
that are available after the trajectory has been processed. Douglas-Peucker
selects a subset of the original trajectory and stores them as its compressed
version. There is no decoding step that reconstructs the original values. In
contrast, the autoencoder compresses the original trajectory into a
lower-dimensional representation that is decoded afterwards. The reconstructed
trajectory contains the same number of time steps as the original but since the
compression is lossy, the reconstructed values are no subset of the original
time series. The latent variable itself can't be used for comparison since the
correlations between the original data and the compressed data are not obvious.

As the compression ratio is set for both methods, the performance can be
evaluated by computation of the distance between the original trajectory and
the compression or reconstruction respectively. Since there is no distance
metric that is meaningful for each use case, multiple metrics are employed for
comparison:

\begin{itemize}
	\item Mean Euclidean/haversine distance (point-to-point)
		\item Fr\'echet distance
		\item Dynamic Time Warping (Dependent)
\end{itemize}

The point-to-point distances have to be further defined for each of the two
datasets, since the Euclidean or haversine distance only measures the distance
between two points in a fixed space. For that reason an aggregate has to be
used to evaluate a trajectory compression.  Furthermore the incorporation of
temporal properties has to be distinguished since the Quake dataset has this
information only implicitly while T-Drive provides it as an additional
value for each data point.

The error calculation for the Quake dataset is straightforward if it is
compressed by the autoencoder. The trajectory is represented as a sequence of
spatial positions in three-dimensional space that are sampled at a fixed rate.
The autoencoder reconstructs each of those points. Therefore the Euclidean
distance between the original and the reconstructed trajectory $T$ and $T'$ is
calculated as the mean of the Euclidean distances between the original points
and their reconstructed counterparts with $n = |T| = |T'|$.

$$
d_{euc}(T, T') =
\frac{1}{n}
\sum_{i=1}^{n}d_{euc}(P_{i}, P'_{i})
\mid P_{i} \in T \land P'_{i} \in T'
$$

If Douglas-Peucker is applied, the compressed trajectory $T'$ is a subset of
the original $T$. Therefore the error of the points that are in both $T'$ and
$T$ is 0 and the points that were removed during compression have to be
approximated by interpolation according to section
\ref{subsec:spatial_distance}. An advantage of the autoencoder model is, that
the temporal information in those trajectories is preserved, since each
sampling point is available after reconstruction. Douglas-Peucker removes
points and the information how many points were removed on the line segments is
lost.

As described in section \ref{subsec:frechet}, the discrete Fr\'echet distance
and Dynamic Time Warping are highly sensitive to the number of sampling
points of both trajectories. For a fair comparison, this number is equalized by
interpolation on the trajectories compressed with Douglas-Peucker. Therefore
it is looked up, how many points have been removed on the line segments of the
compressed trajectory. Those are interpolated linearly on the line segments, so
that both original and compressed trajectory have the same number of points. It
is however important to notice, that this information is only available if the
original trajectory is present and the autoencoder offers a huge improvement in
the reconstruction of every data point. \medbreak

The error calculation becomes more complex if the T-Drive dataset is
compressed. Here the temporal information is represented as an explicit
timestamp at each location which is a popular representation for GPS data. The
previously described approach of simple point-to-point calculation of the
Euclidean distance would entirely discard the temporal information. This data
is also lost, if the trajectory is compressed with standard Douglas-Peucker.
Therefore the Douglas-Peucker variant TD-TR (section \ref{subsec:tdtr}) is used
as a comparison baseline. The main difference between the two alternatives is
the used distance metric. While Douglas-Peucker is based on the perpendicular
distance between points of the original trajectory and the compressed line
segments, TD-TR uses the time dependent Synchronized Euclidean Distance based
on the time-ratio between points. The temporal information is therefore
included in the distance calculation. In order to evaluate the errors of the
T-Drive compression, two scenarios are considered. First, only the spatial
components are compared similar to the comparison with the Quake dataset.
Second, the results of both compression with Douglas-Peucker and reconstruction
with the autoencoder are synchronized in time according to section
\ref{sec:SED}. The distances are afterwards calculated based on points with the
same timestamp, so that the temporal dimension is taken into account.
Furthermore, the Euclidean distance as base metric is exchanged for the
haversine distance.

\section{Implementation}
The proposed model was implemented with Keras (\cite{Chollet2015}). Keras
offers a high-level API that allows fast prototyping of and experimentation
with neural networks. It was chosen to test a variety of different scenarios
and hyperparameter settings without the necessity to work with low-level
implementation details. Keras works as abstraction layer on top of tensor
manipulation libraries like Theano (\cite{TDT2016}), CNTK (\cite{Seide2016})
and Tensorflow (\cite{Abadi2015}) and is written in Python. As backend,
Tensorflow was chosen due to its state-of-the-art performance, while Theano
would have worked as well. The encoder was implemented as a plain LSTM cell,
taking as input a mini-batch with a fixed number of time steps and producing an
output in the latent space. Here the output dimensionality is defined, which
indicates the compression ratio the model achieves. The decoder consists of
multiple Keras layers. With a \texttt{RepeatVector} layer, the encoded variable
is repeated $|T|$ times, so that the latent vector is fed to the next LSTM
layer at each time step. This decoding LSTM cell has an output dimensionality
of 100 in order to increase the ability to learn hidden features. This
value was not determined empirically but showed the best performance in a
trial-and-error case. In order to get the output at each time step, the
\texttt{return\_sequences} flag is set. The LSTM layer is followed by a
\texttt{TimeDistributed} layer, that allows the application of a shared simple
linear Dense layer with three neurons to reconstruct a data point. As optimizer
the Adam algorithm introduced in \cite{Kingma2014} is used, since it is
recommended by various researchers especially in the context of LSTM networks.
Adam is based on stochastic gradient descent and combines the advantages of
other optimization algorithms like AdaGrad and RMSProp. As hyperparameter the
defaults recommended in \cite{Kingma2014} are used. Those parameters are also
the defaults implemented in Keras.

Custom loss functions are implemented, that take the scale factors obtained
from the normalization step together with the predicted and expected
trajectory. Both trajectories are rescaled before the Euclidean or
equirectangular distances respectively are calculated for each point. The
resulting loss vectors of the mini-batch are then fed into Adam in order to
update the weights of the network.

\section{Experimental Setup}\label{sec:experiments}
The main goal of this thesis is the evaluation whether an autoencoder approach
can be used to compress trajectories and how such a model performs in
comparison to traditional compression algorithms. As described in section
\ref{sec:evaluation}, the autoencoder is compared to Douglas-Peucker variants
as baseline. Since the sequence length of the input trajectories is fixed for
the autoencoder, it should be evaluated, how well the model performs with
different given lengths $|T|$. Therefore, each experiment is performed once
with trajectories containing 20 data points and once containing 40. Another
important property that has to be tested is the performance given different
compression ratios. This leads to a couple of different scenarios that are
tested in the rest of this thesis. Table \ref{table:scenarios_20} shows the
compression ratios that are considered for $|T| = 20$ together with the number
of values in the compressed version. Since each point is three-dimensional, the
original trajectory has 60 values. For the autoencoder the number of compressed
values is the sum of the dimensionality of the latent variable and the
variables needed for offset and rescaling. For Douglas-Peucker it is the
product of the number of points stored in the compression and the
dimensionality of each point.

\begin{table}[htb]
\centering
	\begin{tabular}{ c  c  c  c }
		\toprule
		Compression Ratio & Autoencoder & Douglas-Peucker & Compressed
		Values \\
		\midrule
		2 & 24 + 6 & 10 $\cdot$ 3 & 30\\
		4 & 9 + 6 & 5 $\cdot$ 3 & 15\\
		6$\frac{2}{3}$ & 3 + 6 & 3 $\cdot$ 3 & 9\\
		\bottomrule
	\end{tabular}
	\caption{Scenarios evaluated for sequence length 20.}
	\label{table:scenarios_20}
\end{table}

\begin{table}[htb]
\centering
	\begin{tabular}{ c  c  c  c }
		\toprule
		Compression Ratio & Autoencoder & Douglas-Peucker & Compressed
		Values \\
		\midrule
		2 & 54 + 6 & 20 $\cdot$ 3 & 60\\
		4 & 24 + 6 & 10 $\cdot$ 3 & 30\\
		8 & 9 + 6 & 5 $\cdot$ 3 & 15\\
		10 & 6 + 6 & 3 $\cdot$ 3 & 12\\
		\bottomrule
	\end{tabular}
	\caption{Scenarios evaluated for sequence length 40.}
	\label{table:scenarios_40}
\end{table}

The possible compression ratios that can be compared are limited by two
factors. First, Douglas-Peucker selects a subset of the original trajectory,
therefore the number of values in the compressed trajectory has to be divisible
by 3. Second, the proposed autoencoder model transfers the rescale variables
together with the latent variable, therefore the number of values in the
compressed trajectory has to be greater than 6. In order to evaluate the
performance of the autoencoder with higher compression ratios, the sequence
length $|T| = 40$ is also considered, which allows the scenarios shown in table
\ref{table:scenarios_40}.

For each of those scenarios a new model is trained. Since the two datasets
presented in section \ref{sec:datasets} are structurally different and
different loss functions have to be used, the models have to be trained and
tested with both datasets independently. This results in 14 scenarios that are
evaluated. For each of those scenarios, the test dataset is also compressed
with Douglas-Peucker and TD-TR respectively. The errors between the original
and the compressed/reconstructed trajectories are subsequently calculated for
the three considered metrics. The results of those evaluations and an
interpretation are presented in the following chapter.


==> text/Preliminaries.tex <==
\section{Basics}\label{sec:Preliminaries}

\subsection{Spatio-Temporal Trajectories}
Generally, a trajectory describes the path of an object moving in space. In a real-world environment, the trajectory of a moving object is usually recorded at a given sampling rate. 
% Hence, the trajectory of a moving object between this records can only be approximated, normally by using linear interpolation between two consecutive points. 
% A common visualization of a trajectory is therefore a polyline, where the recorded samples are used as
vertices of line segments.

In case of GPS, a sampled data point $P$ is defined as a triple $(x, y, t)$ representing
the position at longitude $x$, latitude $y$ at times $t$.
A spatio-temporal trajectory $T$ is then defined as a sequence of points: $$P_i(x_i, y_i, t_i) \mid i\in{1,2,...,|T|}$$ where $|T|$ is the sequence length. 
% Since these points are recorded one after another, the timestamps inside a trajectory are continuously increasing.

To compare the similarity between two trajectories, appropriate distance metrics have to be defined. 
% One can use the Euclidean distance between points of the trajectories, which are described by two- or three-dimensional Cartesian coordinates.

GPS coordinates of a point are represented by latitude and longitude on the geographic coordinate system. 
To calculate the distance between two GPS records $P=(\varphi, \lambda)$ and
$P'=(\varphi', \lambda')$, the haversine formula is commonly used under the
assumption that the earth can be approximated as a sphere:
\begin{gather*}
 d_{hav}(P, P') = \\
2r\arcsin 
\biggl(
\sqrt{
	\mathrm{hav}(\varphi'-\varphi) +
	\cos(\varphi)
	\cos(\varphi')
	\mathrm{hav}(\lambda'-\lambda)
}
\biggr)
\end{gather*} 
Here $(\varphi, \lambda)$ is the latitude and longitude of point $P$ in
radians, $r$ is the earth's radius and $\mathrm{hav}(z)$ is the haversine
function:

$$
\mathrm{hav}(z) =
\sin^{2}\biggl(\frac{z}{2}\biggr)
$$

If both trajectories are of same size, point-to-point distances, e.g. mean Euclidean distance, can be calculated. Since GPS trajectories also include time information, Meratnia and de By (2004) introduced the
\textit{synchronized Euclidean distance (SED)}, which measures the distance
between spatial points that are synchronized in time. To use this metric, the
temporal information must also be interpolated between two discrete points in
addition to the spatial information \cite{Meratnia2004}. 

Another common metric for trajectory similarity is the Fr\'echet distance, which can be described as follows: a dog and its owner are connected by a
leash while walking along on two different curves. Both can speed up and slow down but they are not allowed to go backwards. In this analogy, the Fr\'echet distance is the length of the
shortest leash that is sufficient to walk with the dog. Since a GPS trajectory is not a continuous curve but rather a polyline, a variant called \textit{discrete Fr\'echet distance} can be used, that just takes the vertices of two poly lines into account. A dynamic programming approach for this metric is shown by Eiter and Mannila \cite{Eiter1994}.

Dynamic time warping (DTW) \cite{Vintsyuk1968} is also commonly applied as similarity metric in this context. In contrast to the Fr\'echet distance, not
the maximum of the minimum distances is used as a similarity measure, but the
sum of the minimum distances. Shokoohi-Yekta et al. (2015 define two different interpretations
of DTW for multi-dimensional time series: dependent dynamic time warping (DTW$_D$) and independent dynamic time warping (DTW$_I$). The latter is defined as the sum of the independently calculated DTW
distances of all dimensions $m \in M$:

$$DTW_{I}(T, T')=\sum^{M}_{m=1}{DTW(T_{m},T'_{m})}$$

In comparison, DTW$_D$ works like the one-dimensional DTW, but the metric that measures the distance has to incorporate all dimensions. Since temporal information is included through time-synchronization, only
the distances of spatial components are relevant \cite{Shokoohi-Yekta2015}. 

\subsection{Autoencoders}
Autoencoders are introduced by Rumelhart et al. (1985) as a solution for
unsupervised learning \cite{Rumelhart1985}. They are described by Kramer (1991) as a
non-linear variant of principal component analysis (PCA) and hence, they can be used for dimensionality reduction \cite{Kramer1991}. In its simplest form, an autoencoder is a multi-layer perceptron with one
hidden layer. Both input and output layer are of same dimensionality, with the hidden layer introducing a bottleneck at lower dimensionality.
Autoencoders learn to encode the data in a compressed representation and decode it into a
reconstruction that is as similar to the original as possible.

A basic autoencoder network takes an input vector $x$ and maps it to a
representation $z$ in the latent space (encoder): $$z = \sigma(Wx + b)$$
Here $\sigma$ is an activation function (e.g. sigmoid or $tanh$), with $W$ as weight and the bias $b$. 
The approximated output is then reconstructed by mapping the
latent representation back into the original dimensionality (decoder): $$x' = \sigma(W'z + b')$$ where $W'$ and $b'$ are the weights and bias of the decoder, respectively. 
$W$ and $b$ are optimized by finding values that minimize the difference between input and output (reconstruction error) based on a loss function using an optimizer, usually as some variant of stochastic gradient descent (SGD).

\subsection{Recurrent Neural Networks}
Basic neural network architectures, e.g., multi-layer perceptron, assume that
all input is independent of previous or following input. This is a limiting factor, since the processing of real-word data often describes sequential events including temporal dependencies. 
%Hence, basic neural architectures are not able to exploit this crucial information efficiently. 
In contrast, recurrent neural networks (RNN) maintain a hidden state over multiple time steps, while reusing the same weight matrix for each input.

Given an input $x^t$ at time $t$, a RNN computes its hidden state at each time
step: $$h^t = f(Ux^t, Wh^{t-1})$$ where $f$ is the state transition function, $U$ is the weight matrix regarding the input and $W$ is the weight matrix regarding the state transition. Since
the hidden state from the past input $h^{t-1}$ is an input to the new hidden
state, temporal information can be captured. The output $y^{t}$ at each time
step $t$ is computed based on the current hidden state and the output weights
$V$:

$$y^t = g(Vh^t)$$

The function $g$ depends on the use case that the network solves, e.g., \textit{softmax} for a classification task, or an entire fully connected layer in case of larger networks. 
% Depending on the application, the output can be discarded as well. 
% Figure \ref{fig:rnn_unrolled} shows a very basic unrolled RNN, where $\tanh$ is used as activation function and the hidden state is used for the next time step.
Unrolling an RNN in the time dimension leads to a number of hidden layers proportional to the number of input time steps (cf. \ref{fig:rnn_unrolled}).
%However, the weights are shared between the time steps which reduces the number of parameters that have to be trained.
Training this simple RNN with gradient descent and backpropagation through time
may lead to poor results, due to exploding or vanishing gradients \cite{Bengio1994}. These shortcomings make it additionally hard to capture dependencies that stretch over multiple time steps. 

\begin{figure}[htb]
	\centering
	\includegraphics[width=0.45\textwidth]{pictures/preliminaries/rnn_unrolled}
	\caption{Unrolled Recurrent Neural Network.}
	\label{fig:rnn_unrolled}
\end{figure} 

To overcome such problems, Hochreiter and Schmidhuber \cite{Hochreiter1997} introduced an extension to RNN
called \textit{Long Short-Term Memory (LSTM)}. The LSTM architecture consists
of memory cells that retain a hidden state similar to standard RNNs, but extend
the capabilities of RNN by regulation of the information flow between time
steps. This is accomplished by gates that are implemented as neural layers and
an additional cell state that transports the information between steps. The
\textit{forget gate} considers the current input and the last hidden state. It
outputs a matrix with values between 0 and 1 that is multiplied with the
previous cell state $C^{t-1}$ so that it indicates which values decrease and which remain in the cell's memory: $$f^{t} = \sigma(W_{f}x^t + U_{f}h^{t-1} + b_{f})$$ 
Here, $W$ and $U$ represent weight matrices of the input and last hidden state,
respectively. For each gate, the weights and the bias $b$ are trained.
The \textit{input gate} decides which parts of the current input are important
and therefore affect the cell state:

$$i^{t} = \sigma(W_{i}x^t + U_{i}h^{t-1} + b_{i})$$

The input is processed by another neural layer, usually using
hyperbolic tangent as activation function: $$z^{t} = \tanh(W_{z}x^{t} + U_{z}h^{t-1} + b_{z})$$ The output of $z^t$ is a matrix of all possible values that can be included to
the current cell state. The input gate $i^t$ decides to which degree those
candidates are added to the new cell state. This is done by a point-wise
multiplication of $z^t$ and $i^t$. The new cell state $C^t$ is therefore
calculated as follows to forget and add new information (point-wise
multiplication of matrices is notated as $\odot$):

$$C^{t} = C^{t-1} \odot f^{t} + z^{t} \odot i^{t}$$

To compute the output of the current step, the input and the hidden
state is processed by another gate: $$o^{t} = \sigma(W_{o}x^{t} + U_{o}h^{t-1} + b_{o})$$ This \textit{output gate} defines which parts of the activated current cell
state are used to which degree as current output $h^{t}$: $$h^{t} = o^{t} \odot tanh(C^{t})$$ The output $h^t$ and cell state $C^t$ are used as inputs for
the next step together with the input data of the next time step.

==> text/Results.tex <==
\chapter{Results}\label{sec:results}
In this chapter the experimental scenarios described previously are evaluated.
The performance of the proposed autoencoder compression model is compared to
Douglas-Peucker and its time-synchronized variant as baseline. The goal is to
see, whether the new compression method is viable and where its advantages and
weaknesses are. The experiments compare the performance with different
compression ratios, trajectory lengths and datasets.

\section{Performance on Quake III Dataset}\label{sec:results_quake}
The Quake III dataset was split into a part for training the autoencoder that
consists of roughly 90\% of the data points and a test part containing the
remaining 10\%. For the evaluation, just the test part was compressed with both
methods. This part of the dataset consists of 26,024 trajectories for a
sequence length of 20 three-dimensional positions and 12,907 for a sequence
length of 40 points.

\subsection{Trajectories with Sequence Length 20}
The Quake III test dataset with a sequence length of 20 points was compressed
with compression ratios of 2, 4 and 6$\mathrm{\frac{2}{3}}$ as described in
section \ref{sec:experiments}. The autoencoder model reconstructs the
intermediate compression back to the original sequence length of 20 points,
while Douglas-Peucker yields 10, 5 and 3 points respectively. For the
autoencoder reconstruction the mean Euclidean distance between points can
therefore be calculated intuitively, while the trajectories that are compressed
with Douglas-Peucker have to be interpolated first in order to equalize the
sequence lengths of original and compression. Therefore the removed points are
approximated on the line segments of the compressed trajectory by linear
interpolation. The mean Euclidean distance between all original points and
their reconstructions is afterwards computed and shown in Table
\ref{table:quake_euc_20}.

\begin{table}[htb]
\centering
	\begin{tabular}{ l r r }
		\toprule
		Compression Ratio & Douglas-Peucker & Autoencoder \\
		\midrule
		2 & 1.33 & 1.59 \\
		4 & 4.93 & 4.71 \\
		6$\frac{2}{3}$ & 19.73 & 17.80 \\
		\bottomrule
	\end{tabular}
	\caption{Mean Euclidean Distance for Sequence Length 20 with Quake III
	dataset.}
	\label{table:quake_euc_20}
\end{table}

\begin{figure}[hpbt]
	\centering
	\includegraphics[width=.5\textwidth]{pictures/results/euclidean_20}%
	\caption[Mean Euclidean of Quake III compression with sequence length
	20.]{Mean Euclidean Distance of 20 points long Quake III
	trajectories with tested compression ratios.}
	\label{fig:euclidean_20_quake}%
\end{figure}

Figure \ref{fig:euclidean_20_quake} shows a plot with the values from Table
\ref{table:quake_euc_20}. As can be seen, the autoencoder performs worse than
Douglas-Peucker if the compression ratio is set to 2, but for the higher
compression ratios, the reconstructed points have a slightly lower error if the
new model is applied. An explanation for this may be the way Douglas-Peucker
works. For a compression ratio of 2, half of the points in the compressed
trajectory are exactly the same as in the original data, since Douglas-Peucker
compresses by selecting a subset of the original. Therefore the error is
completely due to the distances between the deleted points and their
interpolated locations on the compressed trajectory. For higher compression
ratios, less points are identical and the distance becomes higher. The
difference between Douglas-Peucker and the autoencoder is all-in-all small and
the tendency over different compression ratios is similar. It has to be noted
however, that the approximated locations can't be interpolated in this way in a
real-life scenario, since the number of deleted points between the compressed
locations can only be calculated if the original trajectory is still available.
The autoencoder model on the other hand reconstructs each point of the
trajectory. Therefore the comparison method is in favor of Douglas-Peucker, but
the autoencoder model still performs better, at least for higher compression
ratios, if the error is measured with mean Euclidean distance.\medbreak

Next to the mean Euclidean distance other error metrics are used to evaluate
the compression performance as presented earlier. In contrast to point-to-point
based distances like the mean Euclidean distance, the discrete Fr\'echet
distance and DTW take a trajectory as a whole into account, so that it is
possible to compare trajectories with different amounts of points. The mean
discrete Fr\'echet distances over the test dataset are presented in Table
\ref{table:quake_frechet_20}

\begin{table}[htb]
\centering
	\begin{tabular}{ l r r }
		\toprule
		Compression Ratio & Douglas-Peucker & Autoencoder\\
		\midrule
		2 & 24.26 & 5.12\\
		4 & 44.87 & 19.59\\
		6$\frac{2}{3}$ & 71.04 & 47.34\\
		\bottomrule
	\end{tabular}
	\caption[Mean Fr\'echet of Quake III with sequence length 20.]{Mean
	discrete Fr\'echet Distance for Sequence Length 20 with Quake III
	dataset.}
	\label{table:quake_frechet_20}
\end{table}

In terms of the discrete Fr\'echet distance, the autoencoder performs
significantly better than Douglas-Peucker across all compression ratios.
However, as explained in section \ref{subsec:frechet}, the discrete Fr\'echet
distance is an approximation of the actual Fr\'echet distance and is sensitive
regarding differences in the number of vertices of the compared polylines. This
can be verified by interpolating the deleted points in the same way as before
for the Euclidean distance.

\begin{table}[htb]
\centering
	\begin{tabular}{ l  r  r }
		\toprule
		Compression Ratio & \shortstack[c]{Douglas-Peucker \\ (Interpolated)} & Autoencoder\\
		\midrule
		2 & 6.00 & 5.12\\
		4 & 15.11 & 19.59\\
		6$\frac{2}{3}$ & 34.55 & 47.34\\
		\bottomrule
	\end{tabular}
	\caption{Mean discrete Fr\'echet Distance with interpolated positions.}
	\label{table:quake_frechet_inter_20}
\end{table}

Table \ref{table:quake_frechet_inter_20} shows the mean discrete Fr\'echet
distance for the reconstruction with the autoencoder model in comparison with
the interpolated trajectories compressed with Douglas-Peucker. While the
autoencoder performs slightly better in terms of Fr\'echet distance for a
compression ratio of 2, it performs worse for the other two ratios. However,
here again the compressed trajectories yielded by Douglas-Peucker had to be
enriched with information from the original trajectory, whereas the
reconstructions from the autoencoder were not manipulated. Figure
\ref{fig:frechet_results} shows the boxplots of the discrete Fr\'echet
distances between the original trajectories and the Douglas-Peucker
compressions (D.-P.), their interpolated variants (Interpolated) and the
autoencoder reconstructions (AE).

\begin{figure}[bht]
	\centering
	\includegraphics[width=\textwidth]{pictures/results/frechet}
	\caption{Boxplot of discrete Fr\'echet distance for Quake III
	with sequence length 20.}
	\label{fig:frechet_results}
\end{figure}

The remaining two metrics introduced in \ref{subsec:dtw} are variants of
Dynamic Time Warping. The Quake trajectories consist of three-dimensional
spatial positions, so that the use of the dependent variant of DTW makes more
sense, since the dimensions are dependent of each other. As explained
previously, DTW has similarities to the Fr\'echet distance and therefore is
also sensitive to different sequence lengths of the compared trajectories. The
mean distances measured with DTWD are shown in Table \ref{table:quake_dtw_20}.

\begin{table}[htb]
	\centering
	\begin{tabular}{ l r r r }
		\toprule
		CR & \multicolumn{2}{c}{Douglas-Peucker} & Autoencoder \\ \cmidrule{2-3}
		& Normal & Interpolated & \\ \midrule
		2 & 135.64 & 23.24 & 31.71 \\
		4 & 316.23 & 77.16 & 90.07 \\
		6$\frac{2}{3}$& 585.33 & 278.45 & 323.83 \\
		\bottomrule
	\end{tabular}
	\caption[Mean DTW distances for Quake III dataset with sequence length
	20.]
	{Mean DTW distances for Quake III dataset with sequence
	length 20. Distances for Douglas-Peucker are
	calculated for the compressed trajectory and the interpolation.}
	\label{table:quake_dtw_20}
\end{table}

The tendency of these results is similar to the discrete Fr\'echet errors.
The distances between the original trajectories and the autoencoder
reconstructions are significantly smaller than the distances between original
and Douglas-Peucker compressions. However the autoencoder approach doesn't
perform better if the points deleted by Douglas-Peucker are interpolated. This
can also be seen in the Figures \ref{fig:frechet_20_plot_quake} and
\ref{fig:dtwd_20_plot_quake}.

\begin{figure}[hpbt]
	\centering
		\subfloat[Mean Fr\'echet distance.]{%
			\includegraphics[width=.5\textwidth]{pictures/results/frechet_20}%
			\label{fig:frechet_20_plot_quake}%
		}
		\subfloat[Mean DTW distance.]{%
			\includegraphics[width=.5\textwidth]{pictures/results/dtwd_20}%
			\label{fig:dtwd_20_plot_quake}%
		}
		\caption{Mean distances for sequence length 20 and compression
		ratios 2, 4, 6$\frac{2}{3}$.}
		\label{fig:distances_20_plots}
\end{figure}

\subsection{Trajectories with Sequence Length 40}
In the previous section, trajectories with a fixed length of 20 positions were
compressed with different ratios and the resulting compressions were compared
to the original data. Next to different compression ratios it is also
interesting to use different trajectory lengths in order to evaluate the
performance of the here proposed autoencoder model. Therefore trajectories with
a sequence length of 40 positions are compressed with different ratios and the
results of the autoencoder and Douglas-Peucker are compared. The higher
sequence length also allows compression with higher compression ratios like 8
and 10. The mean Euclidean distances are shown in Table
\ref{table:quake_euc_40} and Figure \ref{fig:euclidean_40_quake}.

\begin{table}[htb]
\centering
	\begin{tabular}{ l r r }
		\toprule
		Compression Ratio & Douglas-Peucker & Autoencoder\\
		\midrule
		2 & 1.45 & 1.76\\
		4 & 3.82 & 3.75\\
		8 & 14.85 & 13.88\\
		10 & 24.87 & 24.39\\
		\bottomrule
	\end{tabular}
	\caption{Mean Euclidean distance for sequence length 40 with Quake III
	dataset.}
	\label{table:quake_euc_40}
\end{table}

\begin{figure}[hpbt]
	\centering
	\includegraphics[width=.5\textwidth]{pictures/results/euclidean_40}%
	\caption{Mean Euclidean distance for sequence length 40 with Quake III
	dataset.}
	\label{fig:euclidean_40_quake}%
\end{figure}

The tendencies already visible at the lower trajectory lengths can be
replicated for longer trajectories. The autoencoder model performs worse for a
compression to half of the original size, while higher compression ratios
produce similar results with a tendency in favor of the autoencoder. That
implies that the temporal dependencies between the points can be captured for
both sequence lengths equally well. \medbreak

For both Fr\'echet distance and DTW distance, the results for the 40 points
per trajectory are comparable to the lower sequence length. Table
\ref{table:quake_frechet_40} shows the distances for the trajectories
compressed with Douglas-Peucker, their interpolations and the reconstructions
form the autoencoder.

\begin{table}[htb]
	\centering
	\begin{tabular}{ l l r r r }
		\toprule
		& & \multicolumn{2}{c}{Douglas-Peucker} \\ \cmidrule{3-4}
		CR & & Normal & Interpolated & Autoencoder \\ \midrule
		\multirow{2}{*}{2} & Fr\'echet & 30.23 & 7.89 & 7.29 \\
		& DTW & 278.40 & 46.33 & 70.09 \\ \midrule
		\multirow{2}{*}{4} & Fr\'echet & 52.45 & 14.92 & 16.86 \\
		& DTW & 616.59 & 117.36 & 144.79 \\ \midrule
		\multirow{2}{*}{8} & Fr\'echet & 93.36 & 41.03 & 64.98 \\
		& DTW & 1304.55 & 423.59 & 509.51 \\ \midrule
		\multirow{2}{*}{10} & Fr\'echet & 114.63 & 58.32 & 87.33 \\
		& DTW & 1701.29 & 701.62 & 882.43 \\
		\bottomrule
	\end{tabular}
	\caption[Mean Fr\'echet and DTW distances for sequence length 40 with
	Quake III.]{Mean Fr\'echet and DTW distances for sequence length 40 with
	Quake III dataset.}
	\label{table:quake_frechet_40}
\end{table}

For a better comparison, the trajectories compressed with Douglas-Peucker were
again interpolated to the same number of points as the original trajectories.
The results are similar to the observations from the smaller trajectories. The
distances between the originals and the reconstructions from the autoencoder
are far smaller than the ones between original and Douglas-Peucker
compressions. However, the distances between original and interpolated
compressions are significantly lower than the autoencoder errors. This
strengthens the hypothesis that the main advantage of the autoencoder is the
reconstruction of every point of the original trajectory in contrast to the
selection of a subset. Figure \ref{fig:distances_40_plots} shows the mean
Fr\'echet and DTW distances for a sequence length of 40 over the four tested
compression ratios.

\begin{figure}[hpbt]
	\centering
		\subfloat[Mean Fr\'echet distance.]{%
			\includegraphics[width=.5\textwidth]{pictures/results/frechet_40}%
			\label{fig:frechet_40_plot}%
		}
		\subfloat[Mean DTW distance.]{%
			\includegraphics[width=.5\textwidth]{pictures/results/dtwd_40}%
			\label{fig:dtwd_40_plot}%
		}
		\caption{Mean distances for sequence length 40 and compression
		ratios 2, 4, 8, 10.}
		\label{fig:distances_40_plots}
\end{figure}

The distances between the original trajectories and the subsets produced by
Douglas-Peucker increase linearly over the compression ratio for both distance
metrics. The Fr\'echet distance between the original and the autoencoder
reconstruction is less than the distance between original and interpolated
Douglas-Peucker compression for a compression ratio of 2, but for higher
ratios the autoencoder error grows faster. As explained in section
\ref{subsec:frechet}, the Fr\'echet distance is sensitive to outliers, since it
represents the maximum of the minimal distances between points. As the
distance grows faster for the autoencoder reconstruction than for the
interpolated Douglas-Peucker compression, this indicates that the autoencoder
produces more outliers, that have a great distance to the rest of the
trajectory. This observation is supported by figure \ref{fig:dtwd_40_plot},
where the mean DTW distances are shown. The autoencoder distance here is always
higher than the interpolated Douglas-Peucker distance, but the difference
between the two methods grows slower for higher compression ratios compared to
the Fr\'echet distance. Since the DTW distance measures the sum of minimal
distances between points, this metric is not as sensitive to outliers as the
Fr\'echet distance. An explanation for the greater number of points that get
reconstructed with a big error for high compression ratios is the
dimensionality of the latent space. With a trajectory of 40 three-dimensional
points and a compression ratio of 10, the compression has only 12 values. Six
of those values are already reserved for rescaling and offset, so that the
latent space of the autoencoder has a dimensionality of 6. Due to this low
dimensionality it is probably not possible to capture all the temporal
dependencies which leads to inaccurate reconstructions.

\section{Performance on T-Drive Dataset}
The Quake III dataset was chosen to test the proposed autoencoder model because
it consists of solely spatial dimensions while the temporal information is
available only implicitly. This reduces complexity in the evaluation of the
model as the trajectories can be compared directly. However, the goal of this
thesis is also the evaluation of the autoencoder model based on real-life GPS
trajectory data which is why the T-Drive dataset was chosen as a second data
source. The sequence lengths and compression ratios that are compared are the
same as in section \ref{sec:results_quake}. However, in contrast to the Quake
trajectories, the T-Drive data points consist of two-dimensional spatial data
and a temporal annotation. Therefore the three-dimensional Euclidean distance
used as a base metric in the previous evaluation has to be exchanged in order
to incorporate all available information in the comparison. In this section two
approaches are compared. On the one hand is the spatial comparison, that omits
the temporal dimension and is therefore similar to the comparison of the Quake
III dataset. On the other hand, the temporal information can be incorporated by
synchronizing the spatial points in time before the distance calculation is
done. Since the spatial positions in the T-Drive data are represented as
latitude/longitude pairs, the haversine distance is used instead of the
Euclidean distance. The error is therefore expressed as meters instead of the
abstract distance in the Quake III evaluation.

\subsection{Spatial Comparison}
In order to see whether the results observed in the compression of the Quake
III dataset can be reproduced for real-life data, the temporal component of the
T-Drive dataset is not considered for evaluation in this section. However, the
compression is done on the whole three-dimensional trajectories. As in the
previous evaluation, the trajectories compressed with Douglas-Peucker are once
considered directly as a subset of the original data and once with the
interpolated approximations of the deleted points. Table
\ref{table:tdrive_20_spatial} shows the distance errors in meters for a
trajectory length of 20 points, with compression ratios of 2, 4 and
6$\frac{2}{3}$. A plot of the errors over the tested compression ratios can be
seen on the left side in Figure \ref{fig:tdrive_20_errors}.

\begin{table}[htb]
	\centering
	\begin{tabular}{ l l r r r }
		\toprule
		CR & & \multicolumn{2}{c}{TD-TR} & Autoencoder\\ \cmidrule{3-4}
		& & Normal & Interpolated &  \\ \midrule
		\multirow{3}{*}{2} & Haversine & - & 296.06 & 377.35 \\
		& Fr\'echet & 2456.99 & 1241.50 & 927.95 \\
		& DTW & 9475.40 & 5552.74 & 7511.91 \\ \midrule
		\multirow{3}{*}{4} & Haversine & - & 959.15 & 1031.50 \\
		& Fr\'echet & 4295.25 & 2267.64 & 2248.18 \\
		& DTW & 25418.19 & 16410.83 & 19802.17 \\ \midrule
		\multirow{3}{*}{6$\frac{2}{3}$} & Haversine & - & 2039.93 & 2120.31 \\
		& Fr\'echet & 5904.94 & 3534.91 & 3991.58 \\
		& DTW & 43189.90 & 32096.28 & 39004.58 \\
		\bottomrule
	\end{tabular}
	\caption{Mean distance errors for T-Drive dataset with sequence length
	20.}
	\label{table:tdrive_20_spatial}
\end{table}

The mean haversine error of the autoencoder is slightly higher than the mean
distance between the original trajectories and the interpolated compressions of
Douglas-Peucker. This is in contrast to the results of the compression of
20-point trajectories from the Quake III dataset, where the mean Euclidean
distance of the autoencoder was lower for higher compression ratios. However,
the difference between the two compression methods stays stable for all three
tested compression ratios. As in the previous results, the discrete Fr\'echet
and DTWD error of the autoencoder is significantly lower than the error between
original trajectories and the subsets produced by TD-TR. The DTWD error of the
autoencoder is however higher than the error of interpolated TD-TR
compressions. The tendency that the autoencoder performs better than the
interpolated TD-TR compressions for lower compression ratios in terms of
Fr\'echet distance can be replicated for the T-Drive dataset. In summary it can
be said, that the results for both datasets are similar and the performance of
the model introduced in this thesis is not dependent on the compressed
datasets. Figure \ref{fig:tdrive_40_errors} shows the errors for the
compression with sequence length 40. The results are similar to the
observations with 20 points per trajectory. This gives again reason for the
assertion that the model performs equally for both sequence lengths.
Furthermore, the results show that the difference between autoencoder and TD-TR
are smaller for higher compression ratios. This is especially visible for the
mean haversine distance, where the autoencoder performs better with compression
ratios of 8 and 10. In Appendix \ref{appendix:length_20}, a 20-point example
trajectory is shown with its interpolated TD-TR compressions and autoencoder
reconstructions for the considered compression ratios. Appendix
\ref{appendix:length_40} shows another trajectory with 40 points and the
corresponding compressions and reconstructions respectively.

\subsection{Time-Synchronized Comparison}
In the previous section only the spatial dimensions of the trajectories were
considered. Since the data points from T-Drive contain additionally a timestamp
for each position, this information can be included in the performance
evaluation. Since the trajectories compressed with TD-TR are a subset of the
original trajectories, the remaining points are already synchronized in time.
The interpolated compressions and the autoencoder reconstructions however
contain positions that are not synchronized and therefore do not consider the
temporal information. In order to include this additional dimension in the
evaluation, both interpolated TD-TR compressions and autoencoder
reconstructions are synchronized in this section before the errors are
calculated. The resulting distances are shown on the right hand side in Figure
\ref{fig:tdrive_20_errors}.

\begin{figure}[hpbt]
	\centering
		\subfloat[Mean haversine distance.]{%
			\includegraphics[width=.8\textwidth]{pictures/results/haversine_20_tdrive_both}%
			\label{fig:haversine_20_plot_tdrive}%
		}\\
		\subfloat[Mean Fr\'echet distance.]{%
			\includegraphics[width=.8\textwidth]{pictures/results/frechet_20_tdrive_both}%
			\label{fig:frechet_20_plot_tdrive}%
		}\\
		\subfloat[Mean DTW distance.]{%
			\includegraphics[width=.8\textwidth]{pictures/results/dtwd_20_tdrive_both}%
			\label{fig:dtwd_20_plot_tdrive}%
		}
		\caption[Errors of T-Drive dataset for sequence length 20 with
		time-synchronization.]{Mean distances for sequence length 20 and compression
		ratios 2, 4, 6$\frac{2}{3}$ on the T-Drive dataset.
		Trajectories have been time synchronized on the right side.}
		\label{fig:tdrive_20_errors}
\end{figure}

Compared to the results of the solely spatial evaluation, the performance of
both compression methods are different. For TD-TR, the errors are lower if the
interpolated trajectory is synchronized in time before the error calculation.
This is due to the fact, that SED was used as metric to decide which points are
stored in the compressed version. For the autoencoder however, the distances
between original and time-synchronized reconstruction are higher, especially
for low compression ratios. This indicates, that the accuracy of the
reconstruction of the temporal dimension is low and the positions of the
synchronized points are therefore further away from the original positions. A
possible improvement would be a more advanced loss function, that either weighs
the reconstruction error of the timestamp more, or even calculates a
time-synchronized distance.

The results for the time-synchronized error with a sequence length of 40 are
shown on the right hand side of Figure \ref{fig:tdrive_40_errors}. The
observations from the 20-point trajectories and the spatial distances can be
reproduced. The autoencoder performs generally worse than the synchronized
TD-TR compression, but the difference is smaller for higher compression ratios.

\begin{figure}[hpbt]
	\centering
		\subfloat[Mean haversine distance.]{%
			\includegraphics[width=.8\textwidth]{pictures/results/haversine_40_tdrive_both}%
			\label{fig:haversine_40_plot_tdrive}%
		}\\
		\subfloat[Mean Fr\'echet distance.]{%
			\includegraphics[width=.8\textwidth]{pictures/results/frechet_40_tdrive_both}%
			\label{fig:frechet_40_plot_tdrive}%
		}\\
		\subfloat[Mean DTW distance.]{%
			\includegraphics[width=.8\textwidth]{pictures/results/dtwd_40_tdrive_both}%
			\label{fig:dtwd_40_plot_tdrive}%
		}
		\caption[Errors of T-Drive dataset for sequence length 40 with
		time-synchronization.]{Mean distances for sequence length 40 and compression
		ratios 2, 4, 8 and 10 on the T-Drive dataset.
		Trajectories have been time synchronized on the right side.}
		\label{fig:tdrive_40_errors}
\end{figure}


